Expanding Versatility of Agile Locomotion through Policy Transitions Using Latent State Representation

This paper proposes the transition-net, a robust transition strategy that expands the versatility of robot locomotion in the real-world setting. To this end, we start by distributing the complexity of different gaits into dedicated locomotion policies applicable to real-world robots. Next, we expand the versatility of the robot by unifying the policies with robust transitions into a single coherent meta-controller by examining the latent state representations. Our approach enables the robot to iteratively expand its skill repertoire and robustly transition between any policy pair in a library. In our framework, adding new skills does not introduce any process that alters the previously learned skills. Moreover, training of a locomotion policy takes less than an hour with a single consumer GPU. Our approach is effective in the real-world and achieves a 19% higher average success rate for the most challenging transition pairs in our experiments compared to existing approaches.

==> glossary.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{ |p{1.5in}|p{1.2in}|p{3.5in}|} 
        \hline
        \textbf{Name} & \textbf{Math Symbol} & \textbf{Description}\\ \hline
        \hline
        Simulated Agent & & The quadruped robot in a physics-enabled environment controlled through PD-controllers placed at every joint. \\ \hline
        Quadruped robot & & Real-world counterpart of the simulated agent. An A1 quadruped robot that shares the same control interface as the simulated agent. \\ \hline
        Locomotion Gait & & A \emph{periodic} controller that enables legged robots to move. \\ \hline
        Locomotion Policy & $\pi$ & A control policy trained via reinforcement learning to produce a locomotion gait. \\ \hline %  Neural network that controls the PD-target of each joint of the robot/simulated agent. \\ \hline
        Agent's State & $\boldsymbol{s_t}$ & Input of the policy. Includes history of the agent's orientation, joint positions, foot contacts, and past actions. \\ \hline
        Control Parameters & $\boldsymbol{g_t}$ & Another input of the policy. In this work, it's simply the reference motion data at 4 future steps up to 1 second. \\ \hline
        Latent Representation & $\boldsymbol{\psi}$ & Activations of the last hidden layer of a locomotion policy. Encodes a representation of the state of the agent. \\ \hline
        Policy Library & $\Pi$ & A collection of trained locomotion policies. \\ \hline 
        Sim-to-Real & & Deployment of a policy trained in simulation to the real world. \\ \hline
        Domain Randomization & & Randomization of simulation physics parameters during training of a policy to improve sim-to-real performance. \\ \hline 
        Reference Motion & $\{\mathcal M_i\}_{i=1}^{N_\text{refs}}$ & A sequence of keyframes obtained from motion capture data. Each keyframe contains the position and orientation of the root body, and joint angles of each link. \\ \hline
        Policy Switch & & Instantaneous replacement of a currently running policy by another policy. The transition method used in this work. \\ \hline
        Transition & & A method that allows the linking of a pair of policies. See Policy Switch. \\ \hline
        Transition Configuration & $\mathcal{C}=(m, n, \boldsymbol{\psi_m}, \phi_n)$ & A 4-element tuple containing source and destination policies identifiers, source policy's latent representations, and destination phase. Input of the transition function. \\ \hline
        Source Policy Identifier & $m$ & Identifier of the source locomotion policy of a transition. \\ \hline
        Destination Policy Identifier & $n$ & Identifier of the destination locomotion policy of a transition. \\ \hline
        Phase Variables & $\phi \in [0, 1)$ & A scalar that encodes the phase of a locomotion gait. \\ \hline
        Transition Outcome & $\alpha = y$ & A binary value indicating the success of a transition. Ground truth for learning the transition function. \\ \hline
        Transition Function & $f_{\theta}(\mathcal{C})$ & A function that predicts transition success given a transition configuration. Learned with a feedforward neural network. \\ \hline
        Estimated Outcome & $\hat{y}$ & Output prediction of the transition function. \\ \hline
        Neural Meta-Policy & & The strategy used at deployment time to transition between policies available in the library. Queries the transition function to determine appropriate transition time. \\ \hline
    \end{tabular}
\end{table*}


